A surface finite element method for the Navier-Stokes equations on evolving surfaces

We introduce a surface finite element method for the numerical solution of Navier-Stokes equations on evolving surfaces with a prescribed deformation of the surface in normal direction. The method is based on approaches for the full surface Navier-Stokes equations in the context of fluid-deformable surfaces and adds a penalization of the normal component. Numerical results demonstrate the same optimal order as proposed for surface (Navier-)Stokes equations on stationary surfaces. The approach is applied to high-resolution 3D scans of clothed bodies in motion to provide interactive virtual fluid-like clothing.

==> packagesHeader.tex <==
\usepackage[utf8]{inputenc}

\usepackage[
centering,
marginparwidth=0in,
textwidth=6.5in,
marginparsep=2em,
top=2.5cm,
bottom=2.5cm,
%showframe
]{geometry}

\usepackage{graphicx}% Include figure files
\usepackage{dcolumn}% Align table columns on decimal point
\usepackage{bm}% bold math
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{epstopdf, epsfig}
\usepackage{color}
\usepackage{tikz}
\usepackage{pgfplots}
